A Nonlocal diffusion model with $H^1$ convergence for Dirichlet Boundary

In this paper, we present a nonlocal model for Poisson equation and corresponding eigenproblem with Dirichlet boundary condition. In the direct derivation of the nonlocal model, normal derivative is required which is not known for Dirichlet boundary. To overcome this difficulty, we treat the normal derivative as an auxiliary variable and derive corresponding nonlocal approximation of the boundary condition. For this specifically designed nonlocal mode, we can prove its well-posedness and convergence to the counterpart continuous model. The nonlocal model is carefully designed such that coercivity and symmetry are preserved. Based on these good properties, we can prove the nonlocal model converges with first order rate in $H^1$ norm. Our model can be naturally extended to Poisson problems with Robin boundary and corresponding eigenvalue problem.

==> data/experiments.tex <==
\label{sec:experiment}

In this section, we will apply our proposed method on Poisson equation and Laplacian spectra. So far our results are all on the continuous setting. Nevertheless, a natural thinking is to numerically implement such integral model with proper numerical method, where the operators can be approximated by certain discretization technique. Given a proper density of points, one can approximate the integral of a function by adding up the value of the function at each sample point multiplied by its volume weight. Then we can easily discretize each term of our model since there is only integral operator, and result in a linear system.

We perform experiments on two different domain: unit disk in 2D
\[\Omega= \left\{x^2+y^2\leq 1\right\}, \quad \partial \Omega= \left\{x^2+y^2= 1\right\} \]
and upper hemisphere
\[\Omega= \left\{x^2+y^2+z^2=1, z \geq 0 \right\}, \quad \partial \Omega= \left\{x^2+y^2= 1, z=0 \right\}\]

The calculation of the volume weights involves the use of triangulation to construct local mesh around each points. The mesh on the unit disk in generated using Triangle~\cite{shewchuk1996triangle}. It will give us a quality mesh where each triangle has no small or large angles. In \cref{fig:triangle} we provide an illustration of our triangulation, where we only use 100 points on the boundary, which results in 1013 vertices and 1924 triangles totally. Notice that in the following experiments, we put up to 400 points on the boundary, which gives us 20048 vertices and 39694 triangles in total.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/triangle_small.png}
    \caption{Illustration of triangulation of the unit disk.}
    \label{fig:triangle}
\end{figure}
As for the triangulation on the upper hemisphere, we use stereographic projection to project each point on the unit disk to the hemisphere. As the projection preserves angles, we use the same simplices as in unit disk and can get a quality mesh on the hemisphere. The area of of each triangle is then calculated using its three vertices.

After triangulation, we are given the set of points $\left\{p_{i}\right\}_{i=1}^{n} \subset \Omega,\left\{q_{k}\right\}_{k=1}^{m} \subset \partial \Omega$. In addition, we are given the area weight $A_{i}$ for $p_{i} \in \Omega$, and the length weight $L_{k}$ for $q_{k} \in \partial \Omega$. The area weight of $p_{i}$ is calculated as one third of the area sum of all triangles whose vertex contain $p_{i}$. The length weight is just the circumference of unit circle divided by total number of boundary points, i.e. $2\pi/m$. In our experiments, $m=400$ and $n=19648$. We try to choose as many points as possible to eliminate the discretization error.

The kernel functions are chosen as 
\begin{gather*}
    R(r)=e^{-ar}-e^{-a}\\
    \bar{R}(r)=\frac{1}{a}\left(e^{-ar}-e^{-a}\right)-(1-r)e^{-a}\\
    \bar{\bar{R}}(r)=\frac{1}{a^2}\left(e^{-ar}-e^{-a}\right)-\left(\frac{1-r}{a}+\frac{(1-r)^2}{2}\right)e^{-a}
\end{gather*}
where $a$ is a hyperparameter to control the smoothness of kernel function at $r=1$. In the experiments below, we choose $a=5$. 

\subsection{Poisson equation}
The analysis in the previous sections indicates that our integral model \cref{eq:model} can approximate the Poisson equation in quadratic rate. Using the area weight we obtained using triangulation, we can discretize the model into the following linear system:
\begin{equation}
	\left\{\begin{aligned}
		\frac{1}{\delta^2} \sum_{j=1}^n R_{\delta}(p_i, p_j) \left(u_i-u_j\right)A_j -2 \sum_{l=1}^m \bar{R}_{\delta}(p_i, q_l) v_l L_l &=\sum_{j=1}^n \bar{R}_{\delta}(p_i, p_j) f(p_j)A_j, && i=1,\cdots n \\
		\frac{1}{\delta^2} \sum_{j=1}^n \bar{R}_{\delta}(q_k, p_j) \left(b_k-u_j \right)A_j- 2 \sum_{l=1}^m \bar{\bar{R}}_{\delta}(q_k, q_l) v_k L_l &=\sum_{j=1}^n \bar{\bar{R}}_{\delta}(q_k, p_j) f(p_j)A_j, && k=1,\cdots m
	\end{aligned}\right.
	\label{eq:linear_model}
\end{equation}
in which $u_i=u_{\delta}(p_i), v_k=v_{\delta}(q_k), b_k=b(q_k)$.

We solve the linear system \cref{eq:linear_model} to get $(u_i,v_k)$, and compare with the ground truth value $(u, \frac{\partial u}{\partial \mathbf{n}})$ at each point. Since the $H^1$ norm is hard to calculate, we compute $L^2$ norm for both interior and boundary errors, as defined below.

\begin{gather*}
    \text { Interior } L^{2} \text { error }=\sqrt{\sum_{i=1}^{n}\left(u_{i}-u\left(p_{i}\right)\right)^{2} A_{i}}, \\
    \text { Boundary } L^{2} \text { error }=\sqrt{\sum_{k=1}^{m}\left(v_{k}-\frac{\partial u}{\partial \mathbf{n}}\left(q_{k}\right)\right)^{2} L_{k}}.
\end{gather*}

\subsubsection{Unit disk}
Our model is tested on both homogeneous and nonhomogeneous functions. We range $\delta$ from 0.03 to 0.50, with step size 0.01. We take logarithm on both errors and $\delta$, and use linear regression to get the convergence rate of interior/boundary error with $\delta$. We test with homogeneous function $u(x,y)=r^2-r^4$, and nonhomogeneous function $u(x,y)=r^2-2r^4$, where $r$ is defined as $\sqrt{x^2+y^2}$. To eliminate the effect of discretization, we choose 
$(m,n)=(300,9730),(400,19615),(600,39361)$ in the unit disk and on the boundary, reporting the interior and boundary convergence rate for each discretization density, respectively.

\begin{table}[H]
	\centering
	\begin{tabular}{ccccc}
		\toprule
		$u(x,y)$ & $(m,n)$ & Interior rate & Boundary rate \\
		\midrule
		\multirow{3}{*}{$r^2-r^4$} & $(300,9730)$ & 1.58 & 0.73 \\
		& $(400,19615)$ & 1.50 & 0.71 \\
	    & $(600,39361)$ & 1.45 & 0.69 \\
		\hline 
		\multirow{3}{*}{$r^2-2 r^4$} & $(300,9730)$ & 1.84  & 0.85 \\
		& $(400,19615)$ & 1.71  & 0.81 \\
		& $(600,39361)$ & 1.62  & 0.78 \\
		\bottomrule
	\end{tabular}
	\caption{The convergence rate of functions.}
	\label{table:2d_dirichlet}
\end{table}

\begin{figure}[H]
    \centering
    \subfloat[Interior $L^2$ error]{\includegraphics[width=0.48\linewidth]{figures/cfg_4-8_interior.png}}
    \hfill
	\subfloat[Boundary $L^2$ error]{\includegraphics[width=0.48\linewidth]{figures/cfg_4-8_boundary.png}}
    \caption{Convergence rate for $u=r^2-r^4$. $x$-axis represents $\log(\delta)$, $y$-axis represents $\log(\mathrm{error})$. $(m,n)=(300,9730),(400,19615),(600,39361)$ correspond to coarse, normal and dense legend in the plot.}
    \label{fig:2d_dirichlet}
\end{figure}
The convergence rate of function $u=r^2-r^4$ is described in \Cref{fig:2d_dirichlet}. One may notice that when $\delta$ is too small, the convergence rate is not optimal. When $\delta$ is too small, the neighborhood contains too few points, which makes the discretization error dominant. \cite{shi2017convergence} gives an analysis of discretization error, where $\delta$ lies on the denominator. Thus the smaller $\delta$ is, the larger the discretization error.
% When $\delta$ is too large, the problem arises from our assumption that $\delta \rightarrow 0$. We need $\delta$ sufficiently small to complete the proof.

% Moreover, we try to solve Poisson equation with Robin boundary condition as in \cref{sec:robin}. The corresponding linear model is a discretization of \cref{eq:model_robin}, which is similar to the procedure before. We test on function $u=\sin(\frac{3}{4} \pi r^2)$, and consequently $\mu=\frac{2}{3\pi}$. The interior and boundary convergence rate is 1.42 and 1.14, respectively. The figure is given in~\cref{fig:2d_robin}.

% \begin{figure}[H]
%     \centering
%     \subfloat[$y=1.42x+1.63$]{\includegraphics[width=0.48\linewidth]{figures/interior_robin_2d_cfg_2.png}}
%     \hfill
% 	\subfloat[$y=1.14x+2.77$]{\includegraphics[width=0.48\linewidth]{figures/boundary_robin_2d_cfg_2.png}}
%     \caption{Convergence rate for $u=\sin(\frac{3}{4} \pi r^2)$. (a) Interior $L^2$ error (b) Boundary $L^2$ error.}
%     \label{fig:2d_robin}
% \end{figure}

\subsubsection{Hemisphere}
Other than the unit disk, we conduct experiments on the upper hemisphere in 3D. Using spherical coordinates, the Laplace operator on the sphere can be expressed as
\[\Delta f = \frac{1}{\sin \theta} \frac{\partial}{\partial \theta}\left(\sin \theta \frac{\partial f}{\partial \theta}\right)+\frac{1}{\sin ^{2} \theta} \frac{\partial^{2} f}{\partial \varphi^{2}} \]

The other procedures are identical to that of unit disk, and we also pick homogeneous function homogeneous function $u(x,y,z)=z^2$ and nonhomogeneous function $u(x,y,z)=x$
to test the convergence rate. The results are reported in \Cref{table:3d}. Plot for $u(x,y,z)=z^2$, where $f=-\Delta u=-2+6z^2$, is given in \Cref{fig:3d}.

\begin{table}[H]
	\centering
	\begin{tabular}{ccccc}
		\toprule
		$u(x,y,z)$ & $(m,n)$ & Interior rate & Boundary rate \\
		\midrule
		\multirow{3}{*}{$z^2$} & $(300,9730)$ & 1.60 & 0.71 \\
		& $(400,19615)$ & 1.63 & 0.74 \\
	    & $(600,39361)$ & 1.66 & 0.77 \\
		\hline 
		\multirow{3}{*}{$x$} & $(300,9730)$ & 1.79  & 1.00 \\
		& $(400,19615)$ & 1.80  & 1.03 \\
		& $(600,39361)$ & 1.82  & 1.06 \\
		\bottomrule
	\end{tabular}
	\caption{The convergence rate of functions.}
	\label{table:3d}
\end{table}

\begin{figure}[H]
    \centering
    \subfloat[Interior $L^2$ error]{\includegraphics[width=0.48\linewidth]{figures/cfg_1_interior.png}}
    \hfill
	\subfloat[Boundary $L^2$ error]{\includegraphics[width=0.48\linewidth]{figures/cfg_1_boundary.png}}
    \caption{Convergence rate for $u=z^2$. (a) Interior $L^2$ error (b) Boundary $L^2$ error.}
    \label{fig:3d}
\end{figure}

\subsection{Eigensystem}
In this subsection, we evaluate the effectiveness of our method in calculating the spectra of Laplacian. The integral model is
\begin{equation}
    \frac{1}{\delta^2}\int_{\Omega} R_{\delta}(\mathbf{x}, \mathbf{y})(u_\delta(\mathbf{x})-u_\delta(\mathbf{y})) \mathrm{d} \mathbf{y}+\frac{1}{\delta^2}\int_{\partial \Omega} \frac{\bar{R}_{\delta}(\mathbf{x}, \mathbf{y})}{\bar{\bar{w}}_\delta(\mathbf{y})} \int_{\Omega} \bar{R}_{\delta}(\mathbf{y}, \mathbf{s}) u_\delta(\mathbf{s}) \mathrm{d} \mathbf{s} \mathrm{d} \mathbf{y} = \lambda \int_{\Omega}  \bar{R}_{\delta}(\mathbf{x}, \mathbf{y}) u_\delta(\mathbf{y})\mathrm{d} \mathbf{y}  \label{eq:experiment_eigensystem}
\end{equation}

The discretization procedure is similar as before, approximating the integral of a function by adding up the value of the function at each sample point multiplied by its volume weight. For simplicity, the following results are tested with normal discretization density, i.e. $(m,n)=(400,19615)$. We eventually get a generalized eigenvalue problem.

\subsubsection{Unit disk}
The Laplacian eigenvalue system is also known as Helmholtz equation and has been well studied. On the unit disk, the eigenvalues are the square of $n$-th zero of $m$-order Bessel function $J_{m}(z)$, denoted as $s_{mn}^2$. We compare our results with the first three ground truth eigenvalues other than zero, which are $s_{01}^2= 5.7832, s_{11}^2=14.6820$ and $s_{21}^2=26.3746$~\cite{ismail1982zeros}. The error of eigenvalues is computed as $\left|\lambda - \lambda_{\text{gt}}\right|$. We also derive the error of corresponding eigenvector. The linear system \cref{eq:experiment_eigensystem} gives us a normalized eigenvector $\mathbf{v}$ where $\|\mathbf{v}\|_2=1$. Then we project the eigenvector $v$ onto the space spanned by
\[{J_{m}\left(s_{m n} r\right) \cos (m \theta), \qquad J_{m}\left(s_{m n} r\right) \sin (m \theta)}\]
which is the basis of the eigenspace corresponding to eigenvalue $s_{mn}^2$. The projected vector is called $\mathbf{v}_{\text{gt}}$. Finally we calculate the $L^2$ error of eigenvector as
\[\sqrt{\sum_{i=1}^{n}\left(\mathbf{v}_{i}-\mathbf{v}_{\text{gt},i}\right)^{2} A_{i}}\]

The convergence results are provided in \cref{table:eig_2d} and \cref{fig:eig_2d}. 
\begin{table}[H]
	\centering
	\begin{tabular}{cccc}
		\toprule 
		& $m=0$ & $m=1$ & $m=2$ \\
		\midrule 
		Eigenvalue error & 1.94 & 2.78 & 2.58 \\
		Eigenvector error & 2.08 & 2.08 & 2.00 \\
		\bottomrule
	\end{tabular}
	\caption{The convergence rate of eigenvalues and eigenvectors on unit disk.}
	\label{table:eig_2d}
\end{table}

\begin{figure}[H]
    \centering
    \subfloat[Eigenvalue error]{\includegraphics[width=0.48\linewidth]{figures/eigval.png}}
    \hfill
	\subfloat[Eigenvector error]{\includegraphics[width=0.48\linewidth]{figures/eigvec.png}}
    \caption{Convergence rate for eigenvalue error and eigenvector error for $m=0$.}
    \label{fig:eig_2d}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[$y=1.94x+0.27$]{\includegraphics[width=0.33\linewidth]{figures/eigval_2d_cfg_1.png}}
%     \hfill
% 	\subfloat[$y=2.78x+3.07$]{\includegraphics[width=0.33\linewidth]{figures/eigval_2d_cfg_2.png}}
%     \hfill
% 	\subfloat[$y=2.58x+4.51$]{\includegraphics[width=0.33\linewidth]{figures/eigval_2d_cfg_3.png}}
	
% 	\subfloat[$y=2.08x+4.86$]{\includegraphics[width=0.33\linewidth]{figures/eigvec_2d_cfg_1.png}}
%     \hfill
% 	\subfloat[$y=2.08x-3.98$]{\includegraphics[width=0.33\linewidth]{figures/eigvec_2d_cfg_2.png}}
%     \hfill
% 	\subfloat[$y=2.00x-3.47$]{\includegraphics[width=0.33\linewidth]{figures/eigvec_2d_cfg_3.png}}
%     \caption{(a)(b)(c) Convergence rate for eigenvalue error. ~(d)(e)(f) Convergence rate for eigenvector error.}
%     \label{fig:eig_2d}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/eigval_illustrate.png}
%     \caption{Explanation for the phenomenon in \cref{fig:eig_2d}(b). x-axis: $\delta$, y-axis: $\lambda$, Red line: $\lambda_{\text{gt}}$}
%     \label{fig:eig_illustrate}
% \end{figure}

% The convergence results are provided in \cref{table:eig_2d} and \cref{fig:eig_2d}. The convergence results of eigenvalue for $m=1$ and $m=2$ may seem weird. Actually it is because the computed $\lambda$ pass through the ground truth $\lambda_{\text{gt}}$ as illustrated in \cref{fig:eig_illustrate}.

\subsubsection{Hemisphere}
The eigensystem on the sphere can also be solved analytically. The ground truth eigenvalues are $l(l+1)$ where $l=0,1,2,\cdots$. The corresponding eigenspaces are spanned by the spherical harmonics $Y_l^m(\theta, \phi)$, where $m$ ranges from $-l$ to $l$. We similarly compute the error of eigenvalues and eigenvectors for $l=1,2,3$. The convergence results are provided in \Cref{table:eig_3d}.

\begin{table}[H]
	\centering
	\begin{tabular}{cccc}
		\toprule
		 & $m=0$ & $m=1$ & $m=2$ \\
		\midrule 
		Eigenvalue & 2.14 & 1.66 & 1.39 \\
		Eigenvector & 2.15 & 2.84 & 2.66 \\
		\bottomrule
	\end{tabular}
	\caption{The convergence rate of eigenvalues and eigenvectors on hemisphere.}
	\label{table:eig_3d}
\end{table}

% \begin{figure}[H]
%     \centering
%     \subfloat[$y=2.14x-0.45$]{\includegraphics[width=0.33\linewidth]{figures/eigval_3d_cfg_1.png}}
%     \hfill
% 	\subfloat[$y=1.66x+0.95$]{\includegraphics[width=0.33\linewidth]{figures/eigval_3d_cfg_2.png}}
%     \hfill
% 	\subfloat[$y=1.39x+1.80$]{\includegraphics[width=0.33\linewidth]{figures/eigval_3d_cfg_3.png}}
	
% 	\subfloat[$y=2.15x-5.76$]{\includegraphics[width=0.33\linewidth]{figures/eigvec_3d_cfg_1.png}}
%     \hfill
% 	\subfloat[$y=2.84x-3.81$]{\includegraphics[width=0.33\linewidth]{figures/eigvec_3d_cfg_2.png}}
%     \hfill
% 	\subfloat[$y=2.66x-3.09$]{\includegraphics[width=0.33\linewidth]{figures/eigvec_3d_cfg_3.png}}
%     \caption{(a)(b)(c) Convergence rate for eigenvalue error. ~(d)(e)(f) Convergence rate for eigenvector error.}
%     \label{fig:eig_3d}
% \end{figure}
